Left, Right, and Gender: Exploring Interaction Traces to Mitigate Human Biases

Human biases impact the way people analyze data and make decisions. Recent work has shown that some visualization designs can better support cognitive processes and mitigate cognitive biases (i.e., errors that occur due to the use of mental "shortcuts"). In this work, we explore how visualizing a user's interaction history (i.e., which data points and attributes a user has interacted with) can be used to mitigate potential biases that drive decision making by promoting conscious reflection of one's analysis process. Given an interactive scatterplot-based visualization tool, we showed interaction history in real-time while exploring data (by coloring points in the scatterplot that the user has interacted with), and in a summative format after a decision has been made (by comparing the distribution of user interactions to the underlying distribution of the data). We conducted a series of in-lab experiments and a crowd-sourced experiment to evaluate the effectiveness of interaction history interventions toward mitigating bias. We contextualized this work in a political scenario in which participants were instructed to choose a committee of 10 fictitious politicians to review a recent bill passed in the U.S. state of Georgia banning abortion after 6 weeks, where things like gender bias or political party bias may drive one's analysis process. We demonstrate the generalizability of this approach by evaluating a second decision making scenario related to movies. Our results are inconclusive for the effectiveness of interaction history (henceforth referred to as interaction traces) toward mitigating biased decision making. However, we find some mixed support that interaction traces, particularly in a summative format, can increase awareness of potential unconscious biases.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/old/formative1.tex <==
\section{Formative Study 1}
\label{sec:pilot1}
The goal of this formative study was to understand the bias baseline -- that is, to what degree do things like gender, political party, and so on, impact people's decision making in this scenario? 
In this study, all participants used the \textbf{Control} version of the interface (Section~\ref{sec:system}), described in the previous section, to complete the task (Section~\ref{sec:task}). 
Our hypothesis was that people would focus \textit{explicitly} on 1-2 attributes of the data, while other attributes may be sources of unintentional \textit{implicit} bias.


\subsection{Dataset}
We created a dataset of 144 politicians containing one politician with each combination of \attr{Gender} (Male, Female), \attr{Party} (Republican, Democrat), \attr{Occupation} (Doctor, Lawyer, Business, Career Politician), \attr{Experience} (Low, Medium, High), and the policy view \attr{Ban Abortion After 6 Weeks} (Opposed, Neutral, In Favor). 
Names for each politician were generated based on U.S. census data~\cite{nameGeneratorRef}. 



\subsection{Participants}
We recruited 6 student participants from a large university (3 female, 3 male).
5 participants self-reported that they most identified with the Democratic party, while 1 most identified with the Republican party.
All 6 were opposed to banning abortion after 6 weeks.
We discuss the limitation of participant sampling bias (specifically for political party affiliation) in Section~\ref{sec:discussion}.
Participants self-reported an average of 3.7 out of a 5-point likert scale for familiarity analyzing data using visualizations (1 = least familiar, 5 = most familiar).
We refer to participants from this study as X01-X06. 


\subsection{Results}
Participants rated the importance of attributes that influenced their committee choices on a scale from 1 (least influential) to 7 (most influential). 
Participants indicated that they most explicitly relied on attributes such as the policy view \attr{Ban Abortion After 6 Weeks} ($\mu = 6.3$), \attr{Occupation} ($\mu = 6.2$), \attr{Gender} ($\mu =5.8$), \attr{Experience} ($\mu = 5.7$), and \attr{Party} ($\mu = 5.2$), while ignoring attributes like \attr{First Name} ($\mu = 1.3$) and \attr{Last Name} ($\mu = 1$)~\footnote{While participants claimed to disregard last names, it is possible that name origin could produce unconscious racial bias (e.g.,~\cite{bertrand2004emily}).}.

Many participants intentionally balanced the committee along several attributes (seeking ``balanced representation'' -- X02). 
For example, four participants balanced by \attr{Gender} (5 men and 5 women). 
The same four also balanced by \attr{Party} (5 Republicans and 5 Democrats). 
One participant, X06, intentionally biased heavily toward \attr{Gender} (choosing a committee of 10 women), while attempting to balance other attributes to ``represent different views and backgrounds of women as this is a decision for women to make.''

The ways that participants biased their committee selections were explicit but nuanced. 
While X05 balanced across \attr{Gender} and \attr{Party}, they chose a committee with all 10 members opposed to the bill, explicitly prioritizing ``members (who) were very opposed to the bill.'' 
Similarly, X01 chose a committee of 4 politicians who were opposed to the bill, while only 3 each who were neutral or in favor of the bill (i.e., breaking ties by biasing toward those opposed to the bill), hoping for ``a vote against the abortion bill'' while also seeking a committee that was ``equally balanced amongst those who opposed, neutral, and in favor of the bill.'' 
The same participant (a Democrat) chose more Republicans than Democrats in their committee (6 v. 4). 

When bias was present (in the form of unequal choices across options), it appeared to be the result of participants' explicit choices of give and take rather than implicit or unintentional biases.
One exception became clear in the summative review: X01 said ``oh, that's interesting'' upon realizing they had unintentionally focused on politicians with more \attr{Experience}.
However, this insight was the exception rather than the rule, as most participants seemed unsurprised by the system's accounting of their interactions and committee member selections. 
We hypothesize this may be the result of the relatively low dimensionality of the data (5 attributes) and few choices per attribute (2-4 possible values per attribute) that enabled participants to maintain a reasonable mental bookkeeping of the things they cared about. 
Hence, in the next formative study, we examine higher dimensional data, with the goal of understanding the impact of implicit bias on people's decision making. 

==> sections/old/formative2.tex <==
\section{Formative Study 2}
\label{sec:pilot2}
In Formative Study 1, we found that participants were able to reasonably maintain a mental accounting of their choices in the data and made explicit choices about how to balance or bias the attributes as a result. 
The goal in this formative study was two-fold: (1) to increase the dimensionality of the dataset from the previous study (and hence the level of realism as people have more things to consider when making selections), and (2) to test the effectiveness of an additional intervention (\emph{real-time} interaction traces) toward mitigating potential biases.
To address the latter goal, participants were divided into either a \textbf{Control} or \textbf{Intervention} condition, which dictated which version of the system they used to complete the task. 
All participants still completed two phases of the study: initial committee selection, followed by summative review of interactions and selections, then revised committee selection.
The task and system are the same as those described in Sections~\ref{sec:task} and~\ref{sec:system}.



\subsection{Dataset}
We aimed for greater realism in this study by increasing the dimensionality of the dataset (i.e., people have more features to keep in mind making their decision), and deriving the dataset of fictitious politicians based on distributions found in the 115th US House of Representatives~\cite{congressRef}.
In this version of the dataset, each of 100 fictitious politicians is described by biographical attributes (e.g., \attr{Occupation}, \attr{Religion}, \attr{Experience}, etc) and policy attributes (e.g., each politician's view on issues like \attr{Legalize Medical Marijuana}, etc). 
%Compared to the Study 1 dataset, we increased the cardinality of Occupation to 12 options (compared to 4 options); we provided numerical values for Political Experience (compared to binned ordinal values); we added policy-related attributes for 6 other policies (compared to only Ban Abortion After 6 Weeks) and placed the values on a 7-point ordinal scale; we added attributes for Age, Education, and Religion. 
Policy attributes take on one of seven ordinal values ranging from \textit{strongly opposed} to \textit{strongly in favor} with a \textit{neutral} option. %an integer number $\in$ [-3, 3] representing the \emph{strength} of the policy (1, 2, or 3; 0 is neutral) and \emph{position} (in favor + or opposed -). 
%For example, a politician with -1 toward the policy \attr{Legalize Medical Marijuana} would be somewhat opposed to legalizing medical marijuana.  
Politicians are assumed to primarily vote along party lines, with a 1\% chance of voting against their party and a 5\% chance of a neutral policy (a hypothesized rate). 
For non-neutral policy positions, values were sampled from a distribution of 30\% \textit{somewhat} \{opposed, in favor\}, 50\% \{opposed, in favor\}, and 20\% \textit{strongly} \{opposed, in favor\}, representing our view that more neutral policies are somewhat more likely than more extreme policies, with party-dependent policies being most likely.
%The dataset used in the study was produced by sampling from the distributions described in Table~\ref{table:datasets}, Formative Study 2 column. 



\begin{comment}
\begin{center}
\begin{table}[h!]
\begin{tabularx}{\columnwidth}{p{0.28\columnwidth}p{0.63\columnwidth}}
\textbf{Attribute} & \textbf{Values} \\ \hline
Name & Sampled randomly by gender \\
Gender & Female (28\% if Democrat, 12\% if Republican); Male (72\% if Democrat, 88\% if Republican) \\
Party & Republican (54\%); Democrat (46\%) \\
Occupation & Career Politician (26\%); Military (2\%); Financier (3\%); Business Person (24\%); Judge (7\%); Lawyer (17\%); Educator (11\%); Doctor (3\%); Minister (1\%); Farmer (3\%); Scientist (1\%); Engineer (2\%) [subsample from those frequently listed among 115th US House~\cite{congressRef}] \\
Education & High School (4\%); Associate's Degree (2\%); Bachelor's Degree (25\%); Master's Degree (22\%); PhD (5\%); Medical Degree (4\%); Law Degree (38\%), constrained by occupation \\
Religion & Christian (88\%); Jewish (6\%); Mormon (2\%); Muslim (1\%); Hindu (1\%); Unaffiliated (2\%) \\
Age (years) & Sampled from a normal distribution $\in {[}32, 87{]}$ with $\mu = 58$ years, $\sigma = 10$ years \\
Political Experience (years) & Sampled from a normal distribution with $\mu = 9$ years, $\sigma = 3$ years
\end{tabularx}
\caption{Biographical attributes describing the fictitious politicians in the Study 2 dataset. The distributions are based on those found in the 115th U.S. House of Representatives~\cite{congressRef}, and the names are sampled from U.S. census data~\cite{nameGeneratorRef}. 
}
%\vspace{-4em}
\label{table:bio}
\end{table}
\end{center}

\begin{center}
\begin{table}[t!]
\begin{tabularx}{\columnwidth}{p{0.75\columnwidth}p{0.25\columnwidth}}
\textbf{Attribute (Policy Strength)} & \textbf{Values} \\ \hline
\attr{Legalize Medical Marijuana} & D (+); R (-) \\
\attr{Ban Abortion After 6 Weeks} & R (+); D (-) \\
%\attr{Budget for Free School Lunch Program} & D (+); R (-) \\
\attr{Budget for Free School Lunch} & D (+); R (-) \\
\attr{Increase Gun Control Legislation} & D (+); R (-) \\
\attr{Ban Alcohol Sales on Sundays} & R (+); D (-) \\
%\attr{Increase Budget for Medicare Coverage} & D (+); R (-) \\
\attr{Increase Budget for Medicare} & D (+); R (-) \\
%\attr{Increase Budget for Veterans Affairs (VA)} & D (+); R (-)
\attr{Increase Budget for VA} & D (+); R (-)
\end{tabularx}
\caption{Positions on various policies used to describe the fictitious politicians in the Study 2 dataset. 
R = Republican, D = Democrat. 
(+) indicates typically \emph{in favor of} the policy, while (-) indicates typically \emph{opposed to} the policy.
%\alex{I think we need to bring a little of the commented out text below back in. It wasn't clear at first glance what these + and - are}
%Positive values indicate that the politician is in favor of the bill, while negative values indicate the politician is against the bill. The magnitude of the number represents the strength of their policy (i.e., closer to 0 represents a policy closer to neutral).
}
\label{table:policy}
\end{table}
\end{center}
\end{comment}


\subsection{Participants}
In this study, we recruited 24 participants from a large university (3 female, 21 male). 
21 participants self-reported that they most identified with the Democratic party, and 3 participants most identified with the Republican party.
All participants self-reported at least moderate familiarity with analyzing data using visualizations ($\geq$ 3 out of a 5-point likert scale), with an average of 4.1.
References to specific participants are labeled according to condition (i.e., Y01-C -- Y12-C for Control and Y01-I -- Y12-I for Intervention).





\subsection{Results}
%In this pilot study we sought to understand how visualization of interaction traces might impact decision making in a political scenario. 
We can analyze the bias mitigation strategies with respect to two measures of success, which we refer to as \emph{process} v. \emph{decision}. 
That is, we can measure bias in the user's analysis \emph{process} (using bias metrics~\cite{WallBias}) as well as bias in their final \emph{decision} (by looking at how balanced the political committee is with respect to various attributes of the data).
Data analysis in this study was exploratory in nature. 
Next, we report on the most significant results; however, analysis for all attributes is included in supplemental materials. 
% The following sections address these analyses.





\medskip
\noindent\textbf{Bias in Analysis \emph{Process}. }
We analyze \emph{bias in the analysis process} between the Control and Intervention conditions by comparing the bias metric values~\cite{WallBias}.
Viewed over time, the bias metric values (AD, in particular) can indicate how closely the user's focus on the data analysis was proportional to the underlying data. 
Since the data violates conditions of normality, we analyze participants' bias metric values using the Kruskal-Wallis test by ranks, a non-parametric one-way ANOVA~\cite{kruskal1952use}.

Figure~\ref{fig:distribution} shows the aggregate AD metric values over time for participants in each condition for (a) \attr{Gender} and (b) \attr{Age}. 
Time is shown on the x-axis, while the bias metric is shown on the y-axis (higher values = more bias). 
Orange curves represent the average AD bias metric value for Control participants, while blue curves represent the average AD bias metric value for Intervention participants. 
Some attributes show little noticeable difference between conditions (e.g., \attr{Gender}), while others show a clear distinction (e.g., \attr{Age}).
For \attr{Age} (Figure~\ref{fig:distribution_age}), Control participants (orange) tended to have higher metric values over time than Intervention participants (blue), suggesting that Intervention participants interacted with politicians whose ages were more proportional to the underlying dataset ($\mu_C = 0.857$, $\mu_I = 0.729$, $H = 3.360$, $p = 0.057$). 
%Indeed, we find the mean AD bias metric value for \attr{Age} over time for Control and Intervention participants ($\mu_C = 0.857$, $\mu_I = 0.729$, $H = 3.360$, $p = 0.057$).

To better understand the potential impact of real-time bias mitigation strategies, we examine bias metric values over time in conjunction with user interactions with the interaction trace view (Figure~\ref{fig:teaser}F).
For example, Figure~\ref{fig:intervention_impact} shows high bias metric values over most of the task for AD of \attr{Party} for an Intervention participant. 
%The user exhibits high bias throughout most of the task.
Red vertical lines indicate moments when the user interacted with \attr{Party} in the \textit{real-time} interaction trace view (Figure~\ref{fig:teaser}F). 
After interacting with the interaction trace view, the participant's bias toward \attr{Party} decreases. 
One possible explanation is that the user observed bias in their interactions toward Democratic politicians in the interaction trace visualization and consequently went on to focus on Republicans to reduce the bias.  
This trend is not universally true across all participants and attributes; however, it does demonstrate some promise that the interaction trace view has potential to impact the way that users interact with data. 

\begin{figure}[t]
   \centering
   \subfloat[\attr{Gender} attribute]{
\label{fig:distribution_gender}
\includegraphics[width=.48\columnwidth]{figures/evolution_of_distribution_for_gender_for_avg_participants.png}
}
\subfloat[\attr{Age} attribute]{
\label{fig:distribution_age}
\includegraphics[width=.48\columnwidth]{figures/evolution_of_distribution_for_age_for_avg_participants.png}
}
   \caption{Study 2: Average Attribute Distribution metric values for Control (orange) v. Intervention (blue) participants. Higher values (closer to 1) represent higher bias compared to the distribution of the attribute in the full dataset. There is no clear difference between conditions for \attr{Gender} (a), but Control participants exhibited more bias toward \attr{Age} than Intervention participants (b).}
   \label{fig:distribution}
   \vspace{-1em}
\end{figure}




\medskip
\noindent\textbf{Balance: Bias in Final \emph{Decisions}. }
After reviewing the \textit{summative} interaction trace visualization, 12 participants immediately resubmitted their initial committee. 
Another 5 participants looked back at the data but ultimately made no revisions, and 7 participants (4 C, 3 I) changed members of their committee. 
We describe analyses below from both phases, and discuss this result further in Section~\ref{sec:discussion}. 
%We analyze the \emph{bias in the final decisions} of committee members chosen between the control and intervention conditions.
%For the sake of space, we focus on two particularly salient social biases that may be present in this task: toward political party and toward gender, though analysis of all attributes is present in supplemental materials.

During the study, several participants mentioned some desire to \emph{balance} the committee they selected. 
However, people tended to refer to balance in different ways. 
Many participants thought of a balanced committee as one which has diversity and / or equal representation of values (e.g., Y15-C said, ``I would have preferred to have members from all the religious groups and education levels in the committee.''); whereas others thought of a balanced committee as one which was proportional to the dataset and / or electorate (e.g., Y13-C said, in reference to the criteria for selecting his committee, that they sought ``an accurate representation of the opinions of the people of Georgia''). 
Some people seemed to refer to both notions in conflict. 
For example, upon realizing his chosen committee had 5 men and 5 women, Y09-I observed ``There were more men in the dataset. I chose pretty balanced.''
We further address this multiplicity in balance perspectives in Section~\ref{sec:discussion}. 
Supplemental materials contain analyses for all other attributes of the data, as well as additional ways of quantifying balance (e.g., by notions of \emph{diversity} or \emph{proportionality}).

We use the term \emph{balance} in the context of our analysis to quantify an objective ratio of attribute values. 
For instance, we can discuss the issue of gender balance in the chosen committees by examining the ratio of male politicians chosen in each participant's committee.
Since the data violates conditions of normality, we analyze participants' balance in committees using the Kruskal-Wallis test by ranks, a non-parametric one-way ANOVA~\cite{kruskal1952use}.
We focus herein on \attr{Gender}, based on prior exploratory findings.

We compare Control v. Intervention participants in Phase 1 and in Phase 2 of the study. 
Of all attributes of the data, 9 participants (6 C, 3 I) self-reported that \attr{Gender} was the primary consideration in their decision making. 
Figure~\ref{fig:gender_ratio_pilot_2} shows the ratio of male committee members chosen in Phase 1 (x-axis) and in Phase 2 (y-axis).
% Shape indicates the participant's condition (C or I), and color indicates the participant's gender. 
We find that Intervention participants choose a higher ratio of male committee members than Control participants in Phase 1 of the task ($\mu_C = 0.492$, $\mu_I = 0.683$, $H = 4.795$, $p = 0.029$) as well as in Phase 2 ($\mu_C = 0.492$, $\mu_I = 0.658$, $H = 4.537$, $p = 0.033$).

Many participants thought of a balanced committee as one in which both genders were represented in \emph{equal} numbers (e.g., Y18-C expressed his criteria included ``gender equal'')
However, the bias metrics compare interactions to the underlying \emph{distribution} of the data. 
In the study dataset, 13\% were female politicians, while 87\% were male. 
Thus, while Control participants tend to pursue equal numbers of each gender (Figure~\ref{fig:gender_ratio_pilot_2}, gray), the real-time Intervention was correlated with more male-dominant committee selections, consistent with nudging users toward choices proportional to the underlying distribution of the data (Figure~\ref{fig:gender_ratio_pilot_2}, green). 

\begin{figure}[t]
\centering
\includegraphics[width=0.7\columnwidth]{figures/intervention_impact_party.pdf}
\caption{The Attribute Distribution (\attr{Party}) metric value for one Study 2 Intervention participant. 
Vertical red lines indicate interactions with \attr{Party} in the real-time interaction trace view (Figure~\ref{fig:teaser}F).}
\label{fig:intervention_impact} 
\vspace{-1em}
\end{figure}




\begin{figure*}[t!]
   \centering
   \subfloat[Study 2]{
\label{fig:gender_ratio_pilot_2}
\includegraphics[width=.4\linewidth]{figures/male_ratio_pilot_2.pdf}
}
\hspace{.16cm}
\subfloat[Main Study]{
\label{fig:gender_ratio_main_study}
\includegraphics[width=.4\linewidth]{figures/male_ratio_main_study.pdf}
}
   \caption{The balance of \attr{Gender} in committees chosen by 24 participants in (a) Study 2 and (b) Main Study. Balance is shown as the ratio of men in each participant's chosen committee in Phase 1 (x-axis) and Phase 2 (y-axis), shape-coded by condition and color-coded by participant gender.}
   \label{fig:ratios}
   \vspace{-1em}
\end{figure*}



\begin{comment}
\vspace{0.5em}
\noindent\textit{Political Party. }
5 participants (2 C, 3 I) self-reported that political party was the primary consideration in their decision making. 
Figure~\ref{fig:party_ratio} shows the ratio of Republican committee members chosen in Phase 1 (x-axis) and in Phase 2 (y-axis).
Shape indicates the participant's condition (C or I) and color indicates the participant's preferred political party affiliation. 
In general, participants chose a low ratio of Republican candidates. 
We find no statistically significant difference between the ratio of Republican candidates chosen by control and intervention participants in Phase 1 of the task ($\mu_C = 0.325$, $\mu_I = 0.367$, $H = 0.254$, $p = 0.614$) or in Phase 2 ($\mu_C = 0.333$, $\mu_I = 0.367$, $H = 0.195$, $p = 0.659$).
The common political party imbalances could be due to either (1) bias towards individuals' own political party, or (2) conflicting criteria in committee selection. 
For the latter, it is important to note that the dataset contained only a single female Republican candidate. 
Hence, for those participants who first prioritized gender equality, party equality may have unintended or undesired imbalance. 
We address this limitation in the main study in Section~\ref{sec:study}. 
\end{comment}





\medskip
\noindent\textbf{Qualitative Feedback. }
Participants found the \textit{summative} metric visualization most useful, with a median Likert rating of 4.5 / 5.
They found varying utility in the \textit{real-time} bias metric visualizations (interaction traces): median 4 / 5 for coloring points by DPD; 2 / 5 for AC visualizations; 4 / 5 for AD of numerical attributes; and 3 / 5 for AD of categorical attributes. 
Collectively, this suggest that participants preferred the \textit{summative} metric visualization over the \textit{real-time} metric visualization. 
Of Intervention participants, two did not interact with the interaction trace view at all, two interacted only toward the end of Phase 1, two interacted early on or at random points in the analysis, and 6 interacted many times throughout the decision making process. 

With respect to the increased dimensionality of the dataset from Study 1, we found that participants focused on explicitly balancing or biasing a few attributes, but could not as easily maintain a mental accounting of \textit{all} attributes. 
Several participants indicated frustration as a result (e.g., Y07-I said ``I can only do one thing at a time''). 
Participants expressed more surprise about how their interactions and selections mapped to the underlying dataset when considering the \textit{summative} view, suggesting that the view increased their awareness of bias in their analysis process (e.g., Y10-I said ``I'm surprised I didn't choose a doctor''). 
Some attributes that participants were less focused on had high bias as a result. 
E.g., 0 participants indicated that \attr{Age} was the most important attribute in their decision making; yet, high bias was observed (Figure~\ref{fig:distribution_age}).
However, we see promise in showing interaction traces to increase users' awareness of biases that may be both explicit and implicit.


\medskip
\noindent\textbf{Summary of Findings. }
In this study, we found qualitative evidence that increased dimensionality of the data and cardinality of attribute values resulted in participants' inability to fully explicitly consider. 
We found that showing interaction traces led participants to choose more proportional \attr{Gender} composition in selected committees.
In the case of a dataset with distributions sampled from the U.S. House of Representatives, this means that we encouraged participants in the Intervention condition to ultimately choose more men in their committees. 
We discuss the implications of this result further in Section~\ref{sec:discussion}. 




\begin{comment}
\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/likert/utility_of_summative_metric_view.png}
\caption{Likert ratings (1-5) on the utility of the summative metric view shown after Phase 1 of the study.}
\label{fig:summative_likert} 
\end{figure}


\begin{figure}[t!]
   \centering
   \subfloat[Scatterplot coloring.]{
\label{fig:dpd}
\includegraphics[width=.45\columnwidth]{figures/likert/utility_of_coloring_datapoints_in_scatterplot.png}
}
\hspace{.16cm}
\subfloat[Numerical attribute coverage.]{
\label{fig:ac}
\includegraphics[width=.45\columnwidth]{figures/likert/utility_of_coverage_graph.png}
}
\\
\subfloat[Numerical attribute distribution.]{
\label{fig:ad_numerical}
\includegraphics[width=.45\columnwidth]{figures/likert/utility_of_distribution_graph.png}
}
\hspace{.16cm}
\subfloat[Categorical attribute bar charts.]{
\label{fig:ad_categorical}
\includegraphics[width=.45\columnwidth]{figures/likert/utility_of_bar_charts_cat_attributes.png}
}
   \caption{Likert ratings for the utility of each of the real-time metric visualization components by participants in the intervention condition.}
   \label{fig:real_time_likert}
\end{figure}
\end{comment}

==> sections/old/study.tex <==
\section{Main Study}
\label{sec:study}
The two formative studies (Sections~\ref{sec:pilot1}-\ref{sec:pilot2}) suggested that (1) with relatively low dimensional data, people are effective at maintaining a mental accounting of the data and making explicit choices, and (2) showing interaction traces appears to be a promising way of nudging participants to make choices of \attr{Gender} representation more proportional to the underlying dataset. 
However, analysis in these two studies was exploratory in nature (and thus subject to the forking paths problem~\cite{pu2018garden,gelman2013garden}). 
Furthermore, we sought to address additional limitations incurred in Study 2.
Namely, there was gender bias in our sampling of participants (21 men, 3 women), and the simulated dataset differed from the intended population (U.S. House of Representatives) in a few major ways. 
In this study, we address these concerns in an experiment with pre-planned analyses~\cite{tukey1980we}.



\subsection{System}
We made a few changes to the system for this study. 
In Study 2, beneath the distribution curves, numerical attributes also showed coverage (AC metric~\cite{WallBias}) by visualizing four quartiles of the attribute range (Figure~\ref{fig:teaser}F, bottom), colored according to which have been interacted with (blue) or not (gray). 
In Study 2, participants tended not to notice or use this method of showing interaction traces and found it to be the least useful based on Likert ratings (median 2 / 5). 
Thus, we removed this feature for the main Study. 
We also removed the default selection of the visible attribute in the interaction trace view (so that the distribution comparison is only visible when the user selects an attribute).
Now, if a participant never interacts with the view, we can be sure they did not gain some unmeasurable insight by looking at the default view. 
We also allowed both categorical and numerical attributes to be assigned to axes in the scatterplot (compared to numerical attributes only in Study 2), with data points jittered to prevent overplotting.




\subsection{Dataset}
We sought a balance between the control in the Study 1 dataset and the realism in the Study 2 dataset.
While the distributions in the Study 2 dataset were sampled from the U.S. House of Representatives, there were key differences in the simulated dataset instance we used.
Minor variations included 52 Republicans and 48 Democrats, compared to expected values of 54 and 46. 
More notable differences in the distributions sampled from v. the dataset used in Study 2 included (1) only one female Republican (expected value of 6), (2) no ministers (expected value of one), and no scientists (expected value of one). 
Furthermore, we found that the high dimensionality led users to entirely ignore many attributes. 
In this study, we rectified these differences. 

In this version of the dataset, we generated 144 fictitious politicians. %is described by the attributes in Table~\ref{table:datasets}, Main Study column.
Compared to the Study 2 dataset, we reduced the cardinality of some attributes and removed others, described in detail in supplemental materials. % \attr{Occupation} to 6 options (from 12); we removed \attr{Education} (given that \attr{Occupation} is often highly correlated); we removed all policy-related attributes, except for \attr{Ban Abortion After 6 Weeks}. 
Furthermore, we ensured that the sampled dataset included the appropriate distributions per attribute, including the intersection of \attr{Gender} and \attr{Party}. 


\begin{comment}
\begin{center}
\begin{table}[h!]
\begin{tabularx}{\columnwidth}{p{0.28\columnwidth}p{0.63\columnwidth}}
\textbf{Attribute} & \textbf{Values} \\ \hline
Name & Sampled randomly by gender \\
Gender & Female (28\% if Democrat, 12\% if Republican); Male (72\% if Democrat, 88\% if Republican) \\
Party & Republican (54\%); Democrat (46\%) \\
Occupation & Career Politician (23\%); Business Person (21\%); Lawyer (38\%); Educator (9\%); Doctor (4\%); Scientist (5\%); [subsample from those frequently listed among 115th US House~\cite{congressRef}] \\
Religion & Christian (88\%); Jewish (6\%); Mormon (2\%); Muslim (1\%); Hindu (1\%); Unaffiliated (2\%) \\
Age (years) & Sampled from a normal distribution $\in {[}32, 87{]}$ with $\mu = 58$ years, $\sigma = 10$ years \\
Political Experience (years) & Sampled from a normal distribution with $\mu = 9$ years, $\sigma = 3$ years \\
Ban Abortion After 6 Weeks & \{Opposed (D), Neutral, In Favor (R)\} 
\end{tabularx}
\caption{Attributes describing the fictitious politicians used in the Study 3 dataset. The names are generated based on U.S. census data~\cite{nameGeneratorRef}.
}
\label{table:study3_data}
\end{table}
\end{center}
\end{comment} 


\subsection{Participants}
In this study, we recruited 24 participants from a large university (12 female, 12 male). 
23 participants self-reported that they most identified with the Democratic party, and 1 participant most identified with the Republican party.
All participants self-reported at least moderate familiarity with analyzing data using visualizations ($\geq$ 3 out of a 5-point likert scale), with an average of 4.1.
References to specific participants are labeled according to condition (i.e., Z01-C -- Z12-C for Control participants and Z01-I -- Z12-I for Intervention participants). 




\subsection{Hypotheses}
Based on findings from the previous formative studies, we develop the following hypotheses for the present study:
\begin{itemize}%[nolistsep,noitemsep]
    \item [\textbf{H1}] Intervention participants will exhibit less bias in the \textit{analysis process} than Control participants w.r.t. \attr{Age}.
    \item [\textbf{H2}] 
    Intervention participants will choose more proportional \textit{committee selections} than Control participants w.r.t. \attr{Gender}.
    \item [\textbf{H3}] Participants will use the \textit{real-time} interaction trace view throughout the analysis to keep track of their process. 
%    \item [\textbf{H3.5}] \emily{\textit{Real-time} review of interaction traces will increase \textit{awareness} of bias.}
    \item [\textbf{H4}] \textit{Real-time} review of the interaction traces will impact \textit{interactive behavior}.% toward more proportional choices.
    \item [\textbf{H5}] \textit{Summative} review of interactions and committee selections will increase \textit{awareness} of bias.
    \item [\textbf{H6}] \textit{Summative} review of interactions and committee selections will impact \textit{interactive behavior}.
    \item [\textbf{H7}] Participants will find the \textit{summative} interaction trace view more useful than the \textit{real-time} view.
\end{itemize}





\subsection{Results}

\begin{comment}
\begin{figure*}[p]
\centering
\includegraphics[width=\paperwidth,angle=90]{figures/interactions.pdf}
\caption{A summary of the interactions performed by participants in the control condition (left) and intervention condition (right). \emily{Remove due to space?}}
\label{fig:interactions} 
\end{figure*}
\end{comment}


\noindent\textbf{Bias in Analysis Process. }
%For gender, participants in the Intervention condition tended to have lower average AC bias metric values over time than Control participants ($mu_C = 0.073$, $mu_I = 0.005$, $t = 1.864$, $p = 0.076$); however, participants in both conditions had generally good coverage of the space (and hence low bias metric values). 
Based on results in Study 2, we hypothesized that Intervention participants would exhibit less bias in the analysis process for \attr{Age} than Control participants.
We compare the average AD bias metric value for \attr{Age} over time for Control and Intervention participants. 
We find that Intervention participants have a lower average bias metric value over time; however, the result is not statistically significant ($\mu_C = 0.854$, $\mu_I = 0.784$, $H = 0.013$, $p = 0.908$). 
Hence, our results provide little support for \textbf{H1}. 
%\emily{should we replace Fig.~\ref{fig:distribution_gender} with this graph? so we compare age for Pilot 2 and main Study?}

%- AC mean of gender: $H = 4.965$; $p = 0.026$; $mu_C = 0.073$; $mu_I = 0.005$; everyone generally had high coverage (low bias), but intervention was lower


\medskip
\noindent\textbf{Balance: Bias in Final Decisions. }
While Study 2 results showed significant differences in the final decisions participants made for \attr{Gender} composition of their committees, we do not find a statistical difference in this study with respect to the ratio of men in committees in Phase 1 ($mu_C = 0.492$, $mu_I = 0.467$, $H = 1.565$, $p = 0.211$) or in Phase 2 ($mu_C = 0.458$, $mu_I = 0.467$, $H = 0.430$, $p = 0.512$). 
The ratio of male committee members selected by participants is shown in Figure~\ref{fig:gender_ratio_main_study}.
Thus, our results indicate no support for \textbf{H2}.
8 participants (4 C, 4 I) ultimately chose a balanced committee with respect to \attr{Gender} (5 men, 5 women).
11 others got close to a 50\%-50\% split with a balance of 4 men, 6 women (2 C, 4 I) or 6 men, 4 women (4 C, 1 I). 

\begin{comment}
\vspace{0.5em}
\noindent\textit{Political Party. }
We find similar ratios of Republicans in participants' committees in this study compared to Study 2 in Phase 1 ($mu_C = 0.375$, $mu_I = 0.367$) and Phase 2 ($mu_C = 0.367$, $mu_I = 0.392$), however the differences are not statistically significant.



\vspace{0.5em}
\noindent\textit{Age. }
To analyze participants' choice in committees for age, we divide the age distribution of the dataset into deciles. 
How many deciles did participants' 10-person committees cover? 
We find some difference in Phase 1 ($mu_C = 0.325$, $mu_I = 0.217$, $t = 1.695$, $p = 0.104$), and a slightly greater difference in Phase 2 ($mu_C = 0.333$, $mu_I = 0.233$, $t = 1.787$, $p = 0.088$). 
Participants in the Control condition, in this case, tended to choose committee members that were more dispersed across the range. 
\emily{to do: add vis comparing differences in distributions of Control v. Intervention v. Dataset}
\end{comment}

%- anecdotally, people were biased toward younger politicians; let's plot distribution of age in the dataset over (1) the distribution of committee member choices across control and intervention participants (median age 53 across all participants in phase 1 committee choices [52 C, 53 I]; 59 in phase 2 committee choices [53 C, 53 I]); (2) the distribution of interactions with politicians

%- balance for age: (dividing age into deciles, what proportion was covered by the chosen committee?); phase 2: $t = 1.787$; $p = 0.088$; $mu_C = 0.333$; $mu_I = 0.233$ (people in control condition chose committees that covered more of the space)
%- balance for age: (dividing age distribution into fifths, what proportion was covered by the chosen committee?); phase 1: $t = 2.060$; $p = 0.051$; $mu_C = 0.233$; $mu_I = 0.117$ (people in control condition chose committees that covered more of the space); phase 2: $t = 2.028$; $p = 0.055$; $mu_C = 0.25$; $mu_I = 0.133$


%- User PQ... reported that he chose 4-2-4 in favor-neutral-opposed; but actually chose 5-3-2... might have revised had he realized; didn't pick up on it in summative view either for some reason


\medskip
\noindent\textbf{Effects of \textit{Real-Time} Intervention. }
Only participants in the Intervention condition experienced the \textit{real-time} visualization of interaction traces.
Based on observations in Study 2, we hypothesized that the majority of participants in this study would utilize the interaction trace view (Figure~\ref{fig:teaser}F) throughout their analysis process (similar to Figure~\ref{fig:interactions}A). 
However, three participants never interacted with the interaction trace view, and
%one only interacted once, 
three interacted only at the end of Phase 1 to check their work before submitting (similar to Figure~\ref{fig:interactions}B). 
%and another three interacted at the end to check their work as well as at one other point earlier in the analysis. 
Only two participants utilized the \textit{real-time} interaction trace view throughout their analysis as we anticipated.
Thus, our results indicate no support for \textbf{H3}. 

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/interactions.pdf}
\caption{Interactions performed by two participants in the Intervention condition of the main Study. The x-axis represents time (in discrete interactions). (A) Participant Z10-I interacted with the interaction trace view (distribution\_realtime\_review) throughout their analysis; (B) Participant Z11-I interacted with the interaction trace view only toward the end of Phase 1 of the study, before reaching the \textit{summative} phase (distribution\_summative\_review).}
\label{fig:interactions} 
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/real_time_revisions.pdf}
\caption{The evolving balance of committee choices for (A) \attr{Party} and (B) \attr{Experience}. The dashed vertical line indicates the shift from Phase 1 to Phase 2 of the study. After participants interacted with the \textit{real-time} interaction trace view (blue triangles), the balance of their committee shifted.}
\label{fig:real_time_revisions} 
\vspace{-1em}
\end{figure}



%\emily{todo: insert analysis for H3.5 here if we decide to include it... (regarding real-time awareness)}
%\emily{make sure if we don't code phase 2, we include a sentence about why}
After interacting with the \textit{real-time} interaction trace view, participants often made changes to their selected committee during Phase 1.
Because the interaction trace view compares a user's interactions to the underlying distribution of the data, we hypothesized this would lead to changes in user behavior to \textit{make the committee more proportionally representative of the underlying dataset}. 
By qualitative examination, we find some instances where this is true. 
For example, Figure~\ref{fig:real_time_revisions}A shows how one participant's \attr{Party} balance shifts significantly after examination of the \textit{real-time} interaction trace view for \attr{Party} (blue triangle). 
The participant adjusted the committee from 10 Democrats to 4 Republicans and 6 Democrats. 
In fact, examination of the interaction trace view made the participant aware of a mistake in her analysis: ``I forgot I had only filtered by Democrats.''

While we do see some instances where committees were adjusted to be more proportionally representative, we also see instances where participants adjusted their choices to be more diverse or to be more consistent with pre-existing biases. 
For example, Figure~\ref{fig:real_time_revisions}B shows one participant's balance of \attr{Experience} prior to submitting the initial committee in Phase 1 (dashed vertical line). 
Prior to examining the \attr{Experience} interaction trace view (blue triangle), the participant had only selected politicians with a medium amount of \attr{Experience} ($6 \leq x \leq 10$).
After examination, they added committee members who had high and low \attr{Experience} as well. 
While the majority of politicians fell in the medium \attr{Experience} bin (88/144 $\approx$ 61\%), this participant adjusted toward creating a more diverse committee (4 high, 4 medium, 2 low) rather than one that was proportionally representative. 
Thus, while we do observe participants make adjustments to their committees after using the interaction trace view, there is no clear trend about the \textit{direction} of those adjustments.

In addition to the interaction trace view (Figure~\ref{fig:teaser}F), we also showed interaction traces by coloring points in the scatterplot based on the frequency of user interactions with those points, inspired by the technique described in~\cite{feng2017hindsight}. 
However, different from the results presented in~\cite{feng2017hindsight}, we ultimately observed very little effect on participants' breadth of exploration. 
Since the data is normal, we performed a simple t-test to confirm.
On average, participants in the Intervention condition interacted with more unique data points ($\mu_C = 38.75$, $\mu_I = 41.67$, $t = -0.433$, $p = 0.670$) and interacted more times per data point ($\mu_C = 7.25$, $\mu_I = 8.58$, $t = -0.877$, $p = 0.390$), although the results are not statistically significant. 
Hence, analysis for \textbf{H4} is inconclusive.


\medskip
\noindent\textbf{Effects of \textit{Summative} Interaction Trace View. }
All participants, regardless of condition, were exposed to the \textit{summative} visualization of their interaction traces and committee choices.
We hypothesized that reviewing this \textit{summative} visualization would lead participants to both increased awareness of potential biases, as well as influence their behavior in some cases. 
Before proceeding to the Phase 2 revision, participants were asked to reflect on their observations from the \textit{summative} phase.
Using an open-coding approach, we analyzed participants' videos during the \textit{summative} review phase for indications of \textit{awareness}: statements indicating the participant learned something about their process or selections.
All four authors coded one video and discussed to develop an initial coding. 
Using that coding, all authors again applied that coding to a new video and revised the codes. 
After 3 iterations, we achieved theoretical saturation, and one author proceeded to code the remaining videos according to the \textbf{type of statement} (awareness, reflection, clarification) and the \textbf{object of the statement} (data, interactions, committee, interface-interaction-trace, interface-general, unknown). 
We distinguish \textit{awareness} from \textit{reflection} (statements discussing something the participant already knew about) and \textit{clarification} (questions about the data or interface).
We coded 170 statements, 75 of which were statements about awareness ($\mu = 3.125$ per person). 
22/24 participants spoke at least one statement indicating new awareness about their interactions or selections. 
On average, Control participants made more awareness statements than Intervention participants ($\mu_C = 3.6$, $\mu_I = 2.7$), which we hypothesize may be due to the fact that Intervention participants already saw their interaction traces in \textit{real-time} prior to the summative review phase.
This confirms \textbf{H5}.


However, despite 22/24 participants expressing increased awareness or surprise during the \textit{summative} review phase, only 8 participants (4 C, 4 I) revised their choice of committee in Phase 2 of the study.% (after examining the summative interaction trace view). 
11 participants (7 C, 4 I) interacted more but ultimately chose not to revise, and 5 participants (1 C, 4 I) resubmitted their initial committee without any further interaction.
One reason participants expressed for not revising their committee was concern that making changes along one attribute might unintentionally have an effect on another (Z09-I said ``I didn't realize I focused so much on business people ... But I'll leave it for now because it might mess up balance elsewhere.'').
More Intervention participants immediately resubmitted than Control participants (4 v. 1, respectively), which could suggest that Intervention participants already had increased awareness of how their interactions and selections mapped to the underlying data due to the \textit{real-time} interaction trace views. 
Hence, they may have incorporated that information into their decision making in Phase 1, whereas Control participants only saw this comparison in the \textit{summative} view. 
This provides some support for \textbf{H6}. 

Of the revisions participants made in Phase 2, only two people changed \attr{Gender} composition (perhaps because \attr{Gender} was often an explicit focus in Phase 1).
Comparatively, all 8 participants who revised shifted the distribution of \attr{Occupation} in their selected committee, 5 participants changed the composition of the policy \attr{Ban Abortion After 6 Weeks}, and 4 participants changed the composition of \attr{Party} and \attr{Religion}.
However, as with interactions with the \textit{real-time} interaction trace view, there was no clear trend about the direction in which people revised their committees after looking at the \textit{summative} interaction trace view.
Along different dimensions, participants made revisions that (1) increased the diversity or equal representation of the committee, (2) increased the committee's representativeness of the underlying population in the dataset, or (3) were consistent with the participant's pre-existing biases. 


%- revisions people made: 
%> one participant (C-xr) changed gender distribution between phase 1 and 2 from 7 men, 3 women- to 5 men, 5 women; one participant (C-ZY) increased 5 to 7 women and decreased 5 to 3 men
%> one participant (C-ZY) changed from 8 christians to 7, and added a hindu; one (C-qF) changed from 8 christians to 6, then increased from 2 jews to 3, and added a muslim; one participant (C-xr) reduced from 6 to 5 christians and added a Mormon; one participant (I-Xq) reduced from 8 to 6 christian, increased from 1 to 2 muslim, and added 1 jew
%> one participant (C-Cn) reduced from 3 to 2 lawyers and added an educator; one participant (C-ZY) reduced 3 to 2 educators and added from 2 to 3 lawyers; one participant (C-qF) reduced from 3 to 2 business and from 2 to 1 educator, added a doctor and increased 1 to 2 lawyer; one participant (C-xr) reduced from 2 to 1 business and increased 1 to 2 educator; one participant (I-IC) reduced 3 to 2 business and increased 5 to 6 lawyer; one participant (I-Ms) reduced 4 to 3 lawyer and added a scientist; one participant (I-Xq) reduced 2 to 1 business and increased 1 to 2 doctor; one participant (I-Ya) reduced 4 to 3 lawyer and 3 to 2 career politician, and added a scientist and an educator
%> one participant (C-ZY) removed R and increased 9 to 10 D; one participant (I-IC) increased 4 to 5 R and decreased 6 to 5 D; one participant (I-Xq) decreased 9 to 8 D and increased 1 to 2 R; one participant (I-Ya) increased 5 to 6 R and decreased 5 to 4 D
%> one participant (C-ZY) removed neutral, increased 9 to 10 opposed; one participant (C-qF) increased 3 to 4 neutral and decreased 4 to 3 opposed; one participant (I-Xq) reduced 10 to 8 opposed and added a neutral and an in favor; one participant (I-Ya) increased 5 to 6 in favor and decreased 3 to 2 opposed; one participant (C-xr) increased 2 to 3 neutral and decreased 8 to 7 in favor [to do, check if this participant was in favor of ban or not.]
%> people tended not to change gender distribution as much (probably because that was explicitly a focus from the beginning, so they balanced that early on)


\medskip
\noindent\textbf{Subjective Feedback. }
Overall, participants found the \textit{summative} metric visualization to be quite useful (median Likert rating of 4 / 5).
Real-time interaction trace visualizations were rated a median of 4 / 5 for DPD coloring of scatterplot points and a median of 3.5 / 5 for AD in the interaction trace view.
In line with our findings from Study 2, these results suggest that the \textit{summative} metric visualizations may be more useful to participants than the \textit{real-time} metric visualizations, confirming \textbf{H7}. 
We posit this could be due to participants' preference to focus on the task at hand, then reflect and perform revisions to reduce cognitive load.

\begin{comment}
\emily{remove this paragraph?}
Regarding the dimensionality of the dataset, we observed similar trends as in Study 1 and Study 2. 
Many participants explicitly biased toward particular attributes -- e.g., Z06-C chose a committee of 10 politicians who were opposed to the bill, stating ``no point in making it fair when I have an opinion,'' with similar nuance to these biases (Z06-C later said ``I picked two Republicans who were opposed so it would look more balanced'').
Similarly, Z09-I said, ``I'm inclined to skew it towards women since it's about women's bodies. But that may not be possible from balancing it all,'' then ultimately chose a committee of 5 men and 5 women.
However, compared to Study 2, participants seemed much better able to maintain explicit decision making criteria toward most, but not all attributes, citing lesser surprise about findings during the summative reflection in the study.
\end{comment}

\begin{comment}
\emily{- 1 person (Control) never interacted with filters; 
- 1 participant (Control) interacted with lots of filters and axes initially to familiarize with the data, then left a single configuration to choose all 10 committee members 
- 7 participants (3 C, 4 I) configured the axes initially, and never changed them again; they selected their committee, potentially interacting with filters along the way; 
- and 4 participants (2 C, 2 I) set filters initially and left them for all or most of the analysis, but were more active changing the axes
- whereas, 11 (5 C, 6 I) participants were much more active with both filters and axis changes throughout}
\end{comment}


\begin{comment}
\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/likert/3utility_of_summative_metric_view.pdf}
\caption{Likert ratings (1-5) on the utility of the summative metric view shown after Phase 1 of the study.}
\label{fig:summative_likert_3} 
\end{figure}


\begin{figure}[t!]
   \centering
   \subfloat[Scatterplot coloring.]{
\label{fig:dpd_3}
\includegraphics[width=.45\columnwidth]{figures/likert/3utility_of_coloring_datapoints_in_scatterplot.pdf}
}
\hspace{.16cm}
\subfloat[Interaction Trace View.]{
\label{fig:ad_3}
\includegraphics[width=.45\columnwidth]{figures/likert/3utility_of_interaction_trace_view.pdf}
}
   \caption{Likert ratings for the utility of each of the real-time metric visualization components by participants in the intervention condition.}
   \label{fig:real_time_likert_3}
\end{figure}
\end{comment}


\medskip
\noindent\textbf{Summary of Findings. }
In this study, we addressed two of the primary limitations of Study 2: sampling bias of participants with respect to gender and issues with representation in the dataset.
We addressed these in the context of a study with confirmatory analysis (compared to exploratory analyses in Studies 1 and 2)~\cite{tukey1980we}. 
Our analysis indicates that interaction traces have no statistical effect on participants' \attr{Gender} composition of committee selections. 
%This loss of effect could be the result of many potential factors, which we discuss further in Section~\ref{sec:discussion}.
Nonetheless, qualitative analysis suggests that participants positively viewed the \textit{summative} interaction trace view, which increased participants' awareness of bias and in some cases, impacted their behavior as well.
